A sparse matrix formulation of model-based ensemble Kalman filter

We introduce a computationally efficient variant of the model-based ensemble Kalman filter (EnKF). We propose two changes to the original formulation. First, we phrase the setup in terms of precision matrices instead of covariance matrices, and introduce a new prior for the precision matrix which ensures it to be sparse. Second, we propose to split the state vector into several blocks and formulate an approximate updating procedure for each of these blocks. We study in a simulation example the computational speedup and the approximation error resulting from using the proposed approach. The speedup is substantial for high dimensional state vectors, allowing the proposed filter to be run on much larger problems than can be done with the original formulation. In the simulation example the approximation error resulting from using the introduced block updating is negligible compared to the Monte Carlo variability inherent in both the original and the proposed procedures.

==> Figures/Result_plots/Example_2/cdf_statistic/cdf_statistics.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.465\textwidth}
    \centering
    \makebox[\textwidth][c]{\includegraphics[width=4.7cm, height=4.7cm]{Figures/Result_plots/Example_2/cdf_statistic/emp_cdf_t=1.png}}
    \caption{$t=1$}
    \label{fig:ex_2_KS_cdf_t=1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.465\textwidth}
    \centering
    \makebox[\textwidth][c]{\includegraphics[width=4.7cm, height=4.7cm]{Figures/Result_plots/Example_2/cdf_statistic/emp_cdf_t=2.png}}
    \caption{$t=2$}
    \label{fig:ex_2_KS_cdf_t=2}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.465\textwidth}
    \centering
    \makebox[\textwidth][c]{\includegraphics[width=4.7cm, height=4.7cm]{Figures/Result_plots/Example_2/cdf_statistic/emp_cdf_t=3.png}}
    \caption{$t=3$}
    \label{fig:ex_2_KS_cdf_t=3}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.465\textwidth}
    \centering
    \makebox[\textwidth][c]{\includegraphics[width=4.7cm, height=4.7cm]{Figures/Result_plots/Example_2/cdf_statistic/emp_cdf_t=4.png}}
    \caption{$t=4$}
    \label{fig:ex_2_KS_cdf_t=4}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.465\textwidth}
    \centering
    \makebox[\textwidth][c]{\includegraphics[width=4.7cm, height=4.7cm]{Figures/Result_plots/Example_2/cdf_statistic/emp_cdf_t=5.png}}
    \caption{$t=5$}
    \label{fig:ex_2_KS_cdf_t=5}
    \end{subfigure}
    \caption{Empirical cdf of the Kolmogorov-Smirnov statistics at time steps $t=1, \dots 5$. The blue curve is the empirical cdf of the Kolmogorov-Smirnov statistics computed by comparing the optimal ensembles, while the orange curve is the empirical cdf computed by comparing ensembles updated with different updating procedures.}
    \label{fig:ex_2_KS_cdf}
\end{figure*}

==> Figures/Result_plots/Nonlinear/Example_2/results.tex <==

\begin{figure}
  \begin{center}
    \begin{tabular}{ccc}
      \includegraphics[width=5.1cm, height=4.0cm]{Figures/Result_plots/Nonlinear/Example_2/optimal_ensemble_1_t=5.png}
      & ~~
      &
      \includegraphics[width=5.1cm, height=4.0cm]{Figures/Result_plots/Nonlinear/Example_2/block_ensemble_1_t=5.png} \\[-0.2cm]
      (a) & & (b) \\[-0.1cm]
      \includegraphics[width=5.1cm, height=4.0cm]{Figures/Result_plots/Nonlinear/Example_2/optimal_ensemble_2_t=5.png}
      & &
      \includegraphics[width=5.1cm, height=4.0cm]{Figures/Result_plots/Nonlinear/Example_2/block_ensemble_2_t=5.png} \\[-0.2cm]
      (c) && (d)%\\[-0.4cm]
    \end{tabular}
  \end{center}
  \caption{{Non-linear: The reference solution (black) and the observations (red) along one cross section of the grid at time $T=5$. The green lines are the ensemble elements along the same cross section. Figures (a) and (c) show two simulations from the optimal update procedure, while (b) and (d) display two simulations from the block update}}
  \label{fig:ex_2_nonlin}
\end{figure}

==> document_setup.tex <==


\usepackage{geometry}
\geometry{a4paper,margin=3.2cm}
         

\usepackage[utf8]{inputenc}

\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{comment}
\usepackage{tikz}
\usepackage{mathrsfs}
\usepackage{calligra}
\usepackage{mathtools}



\usepackage{pgfplots, pgfplotstable}
\pgfplotsset{width=10cm, compat=1.9}




%\usepackage{filecontents}


\usepackage{subcaption}
\renewcommand\thesubfigure{(\alph{subfigure})}
\captionsetup[figure]{labelfont={bf}, name={Fig.},labelsep=space}
%\captionsetup[subfigure]{labelformat=simple}
%\usepackage[subrefformat=parens,labelformat=parens]{subfig}
%\captionsetup{subrefformat=parens}
%\renewcommand\thesubfigure{\alph{subfigure}}
%\usepackage{mwe}



\usepackage[ruled]{algorithm2e}

\usepackage{float}

\date{}
%\newcommand{\B}{\boldsymbol}

\bibliographystyle{jasa}
\usepackage[numbers, authoryear, round]{natbib}
\usepackage{natbib}


\theoremstyle{definition}
\newtheorem{example}{Example}

\title{A sparse matrix formulation of model-based ensemble Kalman
filter}
\author{Håkon Gryvill and Håkon Tjelmeland\\[0.1cm]
Department of Mathematical Sciences\\
Norwegian University of Science and Technology\\
Trondheim, Norway \\
Emails: hakon.gryvill@ntnu.no; haakon.tjelmeland@ntnu.no}
%\affil{\orgdiv{Department of Mathematical Sciences}, \orgname{Norwegian University of Science and Technology}, \orgaddress{\street{Alfred Getz' vei 1}, \city{Trondheim}, \postcode{7034}, \country{Norway}}}


==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


